Magnetised winds in dwarf galaxies

The origin and the magnitude of the inter-galactic magnetic field is of primordial importance in the global picture of magnetic field evolution, as it is considered to be the missing link between galactic magnetic fields and cluster magnetic fields on much larger scales. We are testing whether dwarf galaxies are good candidates to explain the enrichment of the IGM: after their discs form and trigger galactic dynamos, supernova feedback will launch strong winds, expelling magnetic field lines in the IGM. We have performed MHD simulations of an isolated dwarf galaxy, forming self-consistently inside a cooling halo. Using the RAMSES code, we have for the first time simulated the formation of a magnetised supernova-driven galactic outflow. This simulation is an important step towards a more realistic modelling using fully cosmological simulations. Our simulations reproduce well the observed properties of magnetic fields in spiral galaxies. The formation and the evolution of our simulated disc lead to a strong magnetic field amplification: the magnetic field in the final wind bubble is one order of magnitude larger than the initial value. The magnetic field in the disc, essentially toroidal, is growing linearly with time as a consequence of differential rotation. We discuss the consequence of this simple mechanism on the cosmic evolution of the magnetic field: we propose a new scenario for the evolution of the magnetic field, with dwarf galaxies playing a key role in amplifying and ejecting magnetic energy in the IGM, resulting in what we call a "Cosmic Dynamo" that could contribute to the rather high field strengths observed in galaxies and clusters today.

==> PaxHeader/article.tex <==
17 gid=784332012
18 uid=1861002210
20 ctime=1278674951
20 atime=1278674951
38 LIBARCHIVE.creationtime=1273052479
24 SCHILY.dev=234881027
21 SCHILY.ino=874177
18 SCHILY.nlink=1

